SpecRepair: Counter-Example Guided Safety Repair of Deep Neural Networks

Deep neural networks (DNNs) are increasingly applied in safety-critical domains, such as self-driving cars, unmanned aircraft, and medical diagnosis. It is of fundamental importance to certify the safety of these DNNs, i.e. that they comply with a formal safety specification. While safety certification tools exactly answer this question, they are of no help in debugging unsafe DNNs, requiring the developer to iteratively verify and modify the DNN until safety is eventually achieved. Hence, a repair technique needs to be developed that can produce a safe DNN automatically. To address this need, we present SpecRepair, a tool that efficiently eliminates counter-examples from a DNN and produces a provably safe DNN without harming its classification accuracy. SpecRepair combines specification-based counter-example search and resumes training of the DNN, penalizing counter-examples and certifying the resulting DNN. We evaluate SpecRepair's effectiveness on the ACAS Xu benchmark, a DNN-based controller for unmanned aircraft, and two image classification benchmarks. The results show that SpecRepair is more successful in producing safe DNNs than comparable methods, has a shorter runtime, and produces safe DNNs while preserving their classification accuracy.

==> algorithms/attack.tex <==
\begin{algorithm}[H]
    \DontPrintSemicolon
    \SetKwFunction{DeepOpt}{DeepOpt}
    \SetKwFunction{Rep}{rep}
    \SetKwFunction{BuildSatisfactionFunction}{construct\_fsat}
    \SetKwFunction{OptimizeSHGO}{shgo}
    \SetKwFunction{GetBoundsByPeaks}{get\_peak\_bounds}
    \SetKwFunction{SplitBounds}{split\_bounds}
    \SetKwFunction{Flatten}{flatten}
    \SetKwProg{Fn}{Function}{:}{\KwRet}
    \SetKwIF{If}{ElseIf}{Else}{if}{}{else if}{else}{end if}
    
    \KwIn{DNN $N: \mathbb{R}^n \to \mathbb{R}^m$, property $\varphi = (X_\varphi, Y_\varphi)$, iteration count $K$, peak-analysis threshold $\omega$.}
    \KwOut{\unsat\ with counterexample or \unknown}
    current\_bounds $\leftarrow$ $[\vec{c}_{\vec{x}}]$
    \tcp*{$[[(l_1, u_1), \dots, (l_n, u_n)]]$}
    \label{line:init}
    $\fsat$ $\leftarrow$ \text{construct\_fsat}($N, \varphi$)\;
    \label{line:fsat}
    \ForEach{$i \in \{1, \dots, K\}$ \label{line:main_loop}}{%
        \ForEach{b $\in$ current\_bounds}{%
            $\vec{x}^c \leftarrow$ \text{optimize}($\fsat, b$)\;
            
            \If{$\fsat(\vec{x}^c) < 0$
            \label{alg:line:fsat-in-bounds}}{%
                \KwRet{$(\unsat, \vec{x}^c)$}\label{alg:line:return-result}
            }
        }
        
        \ForEach{$b \in$ current\_bounds}{%
            \eIf{$i < \sigma$}{
                $b$ $\leftarrow$ \text{get\_peak\_bounds}($\fsat, b$)\label{alg:ounds_by_peaks}
            }{
                $b$ $\leftarrow$ \text{halve\_bounds}($\fsat, b$)\label{line:split}\;
            }10
        }
    }
    \KwRet{$\unknown$}

    \caption{SpecAttack counter-example generation.}
    \label{alg:deep-opt}
\end{algorithm}

==> figures/figure-query-complexity.tex <==
\begin{figure*}[ht]
    \begin{center}
    \pgfplotsset{every axis plot/.append style={thick}}
    \pgfplotsset{every tick label/.append style={font=\scriptsize}}

    \begin{subfigure}[b]{0.33\textwidth}
        \begin{tikzpicture}
            \begin{axis}[
                title={MNIST, CNN},
                ylabel={Success Ratio (\%)},
                xmin=0.01, xmax=10,
                ymin=-0.1,ymax=1.1,
                xtick={0.001,0.01,0.1,1,10},
                ytick={0, 0.2, 0.4, 0.6, 0.8, 1},
                yticklabel = {
                    \pgfmathparse{\tick*100}
                    \pgfmathprintnumber{\pgfmathresult}
                },
                xmode=log,       
                x dir=reverse, 
                xmajorgrids=true,
                xtick style={draw=none}
            ]
            
            \addplot[Colors-A]
                table [x=adversarial_distance, y expr=\thisrow{num_successful}/\thisrow{num_experiments}, col sep=comma] {data/mnist/results_spec_attack.csv}; \label{spec_attack_targ_mnist}
                
            \addplot[Colors-C,smooth,tension=0.05]
                table [x=adversarial_distance, y expr=\thisrow{num_successful}/\thisrow{num_experiments}, col sep=comma] {data/mnist/results_dl2.csv}; \label{DL2_targ_mnist}
                
            \addplot[Colors-B,smooth]
                table [x=adversarial_distance, y expr=\thisrow{num_successful}/\thisrow{num_experiments}, col sep=comma] {data/mnist/results_fgsm.csv}; \label{FGSM_targ_mnist}
    
            
            \end{axis}
        \end{tikzpicture}\\
        %
        \begin{tikzpicture}
            \begin{axis}[
                ylabel={\# Queries},
                xmin=0.005, xmax=10,
                ymin=0,ymax=1000000,
                xtick={0.01,0.1,1,10},
                xmode=log,       
                ymode=log,
                x dir=reverse, 
                xmajorgrids=true,
                grid style=densely dashed,
            ]
        
             \addplot[Colors-A!40,smooth,thin,name path=SA_max]
                table [x=adversarial_distance, y=nfev(max), col sep=comma] {data/mnist/results_spec_attack.csv}; 
                
            \addplot[Colors-A!40,smooth,thin,name path=SA_min]
                table [x=adversarial_distance, y=nfev(min), col sep=comma] {data/mnist/results_spec_attack.csv};
                
            \addplot[Colors-A,fill opacity=0.2] fill between[of=SA_min and SA_max];
                
            \addplot[Colors-A]
                table [x=adversarial_distance, y=nfev(median), col sep=comma] {data/mnist/results_spec_attack.csv}; \label{spec_attack_targ_mnist}
                
            \addplot[Colors-C!40,smooth,thin,name path=DL2_max]
                table [x=adversarial_distance, y=nfev(max), col sep=comma] {data/mnist/results_dl2.csv}; \label{DL2_targ_mnist}
                
            \addplot[Colors-C!40,smooth,thin,name path=DL2_min]
                table [x=adversarial_distance, y=nfev(min), col sep=comma] {data/mnist/results_dl2.csv}; \label{DL2_targ_mnist}
                
            \addplot[Colors-C,fill opacity=0.2] fill between[of=DL2_min and DL2_max];
    
            \addplot[Colors-C,smooth]
                table [x=adversarial_distance, y=nfev(median), col sep=comma] {data/mnist/results_dl2.csv}; \label{DL2_targ_mnist}
            
            \addplot[Colors-B]
                table [x=adversarial_distance, y=nfev(median), col sep=comma] {data/mnist/results_fgsm.csv}; \label{FGSM_targ_mnist}
    
            
            \end{axis}
        \end{tikzpicture}\\
        %
        \begin{tikzpicture}
            \begin{axis}[
                ylabel={Time (s)},
                xmin=0.005, xmax=10,
                ymin=-10,ymax=300,
                xtick={0.01,0.1,1,10},
                xmode=log,       
                x dir=reverse, 
                xmajorgrids=true,
                grid style=densely dashed,
            ]
            
            \addplot[Colors-A!40,smooth,thin,name path=SA_max]
                table [x=adversarial_distance, y=time(max), col sep=comma] {data/mnist/results_spec_attack.csv}; 
                
            \addplot[Colors-A!40,smooth,thin,name path=SA_min]
                table [x=adversarial_distance, y=time(min), col sep=comma] {data/mnist/results_spec_attack.csv}; \label{DL2_targ_mnist}
                
            \addplot[Colors-A,fill opacity=0.2] fill between[of=SA_min and SA_max];
            
            \addplot[Colors-A]
                table [x=adversarial_distance, y=time(median), col sep=comma] {data/mnist/results_spec_attack.csv}; \label{spec_attack_targ_mnist}
                
                
            \addplot[Colors-C!40,smooth,thin,name path=DL2_max]
                table [x=adversarial_distance, y=time(max), col sep=comma] {data/mnist/results_dl2.csv}; 

            \addplot[Colors-C!40,smooth,thin,name path=DL2_min]
                table [x=adversarial_distance, y=time(min), col sep=comma] {data/mnist/results_dl2.csv}; 

            \addplot[Colors-C,fill opacity=0.2] fill between[of=DL2_min and DL2_max];
    
            \addplot[Colors-C,smooth]
                table [x=adversarial_distance, y=time(median), col sep=comma] {data/mnist/results_dl2.csv}; \label{DL2_targ_mnist}

            \addplot[Colors-B]
                table [x=adversarial_distance, y=time(median), col sep=comma] {data/mnist/results_fgsm.csv}; \label{FGSM_targ_mnist}
    
            
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}
    %
    % CIFAR10
    %
    \begin{subfigure}[b]{0.33\textwidth}
        \begin{tikzpicture}
            \begin{axis}[
                title={CIFAR10, ResNet},
                %ylabel={Success Ratio (\%)},
                xmin=0.01, xmax=10,
                ymin=-0.1,ymax=1.1,
                xtick={0.01,0.1,1,10},
                ytick={0, 0.2, 0.4, 0.6, 0.8, 1},
                yticklabel = {
                    \pgfmathparse{\tick*100}
                    \pgfmathprintnumber{\pgfmathresult}
                },
                xmode=log,       
                x dir=reverse, 
                xmajorgrids=true,
                xtick style={draw=none}
            ]
            
            \addplot[Colors-A]
                table [x=adversarial_distance, y expr=\thisrow{num_successful}/\thisrow{num_experiments}, col sep=comma] {data/cifar10/results_spec_attack.csv}; \label{spec_attack_targ_cifar10}
                
            \addplot[Colors-C]
                table [x=adversarial_distance, y expr=\thisrow{num_successful}/\thisrow{num_experiments}, col sep=comma] {data/cifar10/results_dl2.csv}; \label{DL2_targ_cifar10}
                
            \addplot[Colors-B]
                table [x=adversarial_distance, y expr=\thisrow{num_successful}/\thisrow{num_experiments}, col sep=comma] {data/cifar10/results_fgsm.csv}; \label{FGSM_targ_cifar10}
    
            
            \end{axis}
        \end{tikzpicture}\\
        %
        \begin{tikzpicture}
            \begin{axis}[
                %ylabel={\# Queries},
                xmin=0.005, xmax=10,
                ymin=0,ymax=1000000,
                xtick={0.01,0.1,1,10},
                xmode=log,       
                ymode=log,
                x dir=reverse, 
                xmajorgrids=true,
                grid style=densely dashed,
            ]
            
            \addplot[Colors-A]
                table [x=adversarial_distance, y=nfev(median), col sep=comma] {data/cifar10/results_spec_attack.csv}; \label{spec_attack_targ_cifar10}
                
            \addplot[Colors-C!40,smooth,tension=0.2,,thin,name path=DL2_max]
                table [x=adversarial_distance, y=nfev(max), col sep=comma] {data/cifar10/results_dl2.csv}; \label{DL2_targ_cifar10}
                
            \addplot[Colors-C!40,smooth,tension=0.2,,thin,name path=DL2_min]
                table [x=adversarial_distance, y=nfev(min), col sep=comma] {data/cifar10/results_dl2.csv}; \label{DL2_targ_cifar10}
                
            \addplot[Colors-C,fill opacity=0.2] fill between[of=DL2_min and DL2_max];
                
            \addplot[Colors-C]
                table [x=adversarial_distance,smooth,tension=0.2,y=nfev(median), col sep=comma] {data/cifar10/results_dl2.csv}; \label{DL2_targ_cifar10}
                
            \addplot[Colors-B]
                table [x=adversarial_distance, y=nfev(median), col sep=comma] {data/cifar10/results_fgsm.csv}; \label{FGSM_targ_cifar10}
    
            
            \end{axis}
        \end{tikzpicture}\\
        %
        \begin{tikzpicture}
            \begin{axis}[
                %ylabel={Time (s)},
                xmin=0.005, xmax=10,
                ymin=-10,ymax=250,
                xtick={0.01,0.1,1,10},
                xmode=log,       
                x dir=reverse, 
                xmajorgrids=true,
                grid style=densely dashed,
            ]
            
            \addplot[Colors-A]
                table [x=adversarial_distance, y=time(median), col sep=comma] {data/cifar10/results_spec_attack.csv}; \label{spec_attack_targ_cifar10}
            
            \addplot[Colors-C!40,smooth,tension=0.2,thin,name path=DL2_max]
                table [x=adversarial_distance, y=time(max), col sep=comma] {data/cifar10/results_dl2.csv}; \label{DL2_targ_cifar10}
                
            \addplot[Colors-C!40,smooth,tension=0.2,thin,name path=DL2_min]
                table [x=adversarial_distance, y=time(min), col sep=comma] {data/cifar10/results_dl2.csv}; \label{DL2_targ_cifar10}
                
            \addplot[Colors-C,fill opacity=0.2] fill between[of=DL2_min and DL2_max];
    
            \addplot[Colors-C,smooth,tension=0.2,]
                table [x=adversarial_distance, y=time(median), col sep=comma] {data/cifar10/results_dl2.csv}; \label{DL2_targ_cifar10}
                
            \addplot[Colors-B]
                table [x=adversarial_distance, y=time(median), col sep=comma] {data/cifar10/results_fgsm.csv}; \label{FGSM_targ_cifar10}
    
            
            \end{axis}
        \end{tikzpicture}
    \end{subfigure}
    
    \begin{tabular}{@{}r@{ }l@{}r@{ }l@{}r@{ }l@{}}
     \raisebox{0pt}{\tikz{\draw[fill=Colors-A] (0,0) rectangle ++(3mm,2mm);}} & SpecAttack\hspace{4mm} &
     \raisebox{0pt}{\tikz{\draw[fill=Colors-C] (0,0) rectangle ++(3mm,2mm);}} & DL2\hspace{4mm} &
     \raisebox{0pt}{\tikz{\draw[fill=Colors-B] (0,0) rectangle ++(3mm,2mm);}} & FGSM\hspace{4mm}
    \end{tabular}

    \end{center}
    \caption{\textbf{Robustness attacks}:
    The x-axis shows the median $\ell_{\infty}$ distance (log scale).
    The y-axis respectively shows the success ratio, query complexity, and runtime.
    The plots show untargeted (solid line) and targeted (dashed line) perturbed model queries on CIFAR-10 with ResNet, MNIST with CNN, and ACAS Xu with network $N_{2,2}$.
    The evaluated algorithms are SpecAttack (this work), DL2, and FGSM.
    }
    \label{fig:linf-robustness}
\end{figure*}

==> tables/acasxu-full-repair_old.tex <==
\begin{center}
\begin{tabular}{@{}cc|ccc|ccc|ccc@{}}
\toprule
         &       & \multicolumn{3}{c|}{\textbf{Repair Status}} & \multicolumn{3}{c|}{\textbf{Repair Accuracy}} & \multicolumn{3}{c}{\textbf{Repair MAE}} \\
Spec   & Model       & \tool{ } & DL2        & NR         & \tool{ } & DL2 & NR & \tool{ } & DL2 & NR \\
\midrule
\(\varphi_2\) & \(N_{2,1}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.1}  &  --  & 83.9           &   \textbf{0.22}   &    --  & 2242.6 \\
\(\varphi_2\) & \(N_{2,2}\) & \exsuccess & \exfailure & \exsuccess & \textbf{98.7}  &  --  & 85.1           &   \textbf{0.23}   &    --  & 2279.3 \\
\(\varphi_2\) & \(N_{2,3}\) & \exsuccess & \exsuccess & \exsuccess & \textbf{99.3}  & 93.4 & 83.5           &   \textbf{0.13}   &   6.29 & 2420.6 \\
\(\varphi_2\) & \(N_{2,4}\) & \exsuccess & \exfailure & \extimeout & \textbf{99.5}  &  --  &  --            &   \textbf{0.09}   &    --  &    --  \\
\(\varphi_2\) & \(N_{2,5}\) & \extimeout & \exfailure & \exsuccess &  --            &  --  & \textbf{84.1}  &    --             &    --  & \textbf{2433.8} \\
\(\varphi_2\) & \(N_{2,6}\) & \extimeout & \exfailure & \exsuccess &  --            &  --  & \textbf{85.6}  &    --             &    --  & \textbf{2303.7} \\
\(\varphi_2\) & \(N_{2,7}\) & \exsuccess & \exfailure & \exsuccess & 14.5           &  --  & \textbf{87.0}  &   \textbf{0.15}   &    --  & 1644.8 \\
\(\varphi_2\) & \(N_{2,8}\) & \exsuccess & \exsuccess & \exsuccess & \textbf{99.6}  & 89.5 & 87.3           &   \textbf{0.14}   &   5.97 & 663.6  \\
\(\varphi_2\) & \(N_{2,9}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.8}  &  --  & 88.6           &   \textbf{0.13}   &    --  & 2405.1 \\
\(\varphi_2\) & \(N_{3,1}\) & \exsuccess & \exfailure & \exsuccess & \textbf{98.6}  &  --  & 77.5           &   \textbf{0.27}   &    --  & 6.1    \\
\(\varphi_2\) & \(N_{3,2}\) & \exsuccess & \exfailure & \extimeout & \textbf{99.9}  &  --  &  --            &   \textbf{0.10}   &    --  &    --  \\
\(\varphi_2\) & \(N_{3,4}\) & \exsuccess & \exfailure & \extimeout & \textbf{99.5}  &  --  &  --            &   \textbf{0.10}   &    --  &    --  \\
\(\varphi_2\) & \(N_{3,5}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.5}  &  --  & 84.2           &   \textbf{0.09}   &    --  & 2384.2 \\
\(\varphi_2\) & \(N_{3,6}\) & \exunknown & \exfailure & \exsuccess &  --            &  --  & \textbf{81.8}  &    --             &    --  & \textbf{2387.0} \\
\(\varphi_2\) & \(N_{3,7}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.7}  &  --  & 87.0           &   \textbf{0.11}   &    --  & 2251.7 \\
\(\varphi_2\) & \(N_{3,8}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.7}  &  --  & 87.9           &   \textbf{0.09}   &    --  & 1311.1 \\
\(\varphi_2\) & \(N_{3,9}\) & \extimeout & \exfailure & \exsuccess &  --            &  --  & \textbf{87.2}  &    --             &    --  & \textbf{2442.5} \\
\(\varphi_2\) & \(N_{4,1}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.8}  &  --  & 87.7           &   \textbf{0.11}   &    --  & 1939.3 \\
\(\varphi_2\) & \(N_{4,3}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.4}  &  --  & 87.8           &   \textbf{0.13}   &    --  & 2419.4 \\
\(\varphi_2\) & \(N_{4,4}\) & \exsuccess & \exsuccess & \exsuccess & \textbf{99.5}  & 96.0 & 87.9           &   \textbf{0.10}   &   6.03 & 1090.5 \\
\(\varphi_2\) & \(N_{4,5}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.4}  &  --  & 87.5           &   \textbf{0.08}   &    --  &    2.7 \\
\(\varphi_2\) & \(N_{4,6}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.6}  &  --  & 89.8           &   \textbf{0.07}   &    --  & 1329.1 \\
\(\varphi_2\) & \(N_{4,7}\) & \exsuccess & \exfailure & \exsuccess & \textbf{98.3}  &  --  & 88.9           &   \textbf{0.14}   &    --  & 1996.1 \\
\(\varphi_2\) & \(N_{4,8}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.1}  &  --  & 88.6           &   \textbf{0.16}   &    --  & 584.3  \\
\(\varphi_2\) & \(N_{4,9}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.5}  &  --  & 88.8           &   \textbf{0.06}   &    --  & 2292.2 \\
\(\varphi_2\) & \(N_{5,1}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.5}  &  --  & 87.5           &   \textbf{0.11}   &    --  & 2227.2 \\
\(\varphi_2\) & \(N_{5,2}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.7}  &  --  & 87.6           &   \textbf{0.10}   &    --  & 2438.8 \\
\(\varphi_2\) & \(N_{5,4}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.6}  &  --  & 87.8           &   \textbf{0.09}   &    --  & 405.1  \\
\(\varphi_2\) & \(N_{5,5}\) & \extimeout & \exfailure & \exsuccess &  --            &  --  & \textbf{87.9}  &    --             &    --  & \textbf{749.8}  \\
\(\varphi_2\) & \(N_{5,6}\) & \exsuccess & \exfailure & \extimeout & \textbf{99.5}  &  --  &  --            &   \textbf{0.12}   &    --  &     -- \\
\(\varphi_2\) & \(N_{5,7}\) & \exsuccess & \exfailure & \exsuccess & \textbf{98.4}  &  --  & 88.0           &   \textbf{0.16}   &    --  & 957.7  \\
\(\varphi_2\) & \(N_{5,8}\) & \exsuccess & \exfailure & \exsuccess & \textbf{99.4}  &  --  & 87.7           &   \textbf{0.11}   &    --  & 382.5  \\
\(\varphi_2\) & \(N_{5,9}\) & \exsuccess & \exfailure & \exsuccess & \textbf{98.1}  &  --  & 87.9           &   \textbf{0.13}   &    --  & 181.2  \\
\(\varphi_7\) & \(N_{1,9}\) & \exunknown & \exfailure & \extimeout &  --  &  --  &  --  &    --  &    --  &     -  \\
\(\varphi_8\) & \(N_{2,9}\) & \extimeout & \exfailure & \exunknown &  --  &  --  &  --  &    --  &    --  &     -- \\
\(\Phi_1\)    & \(N_{2,9}\) & \extimeout & \exfailure & \extimeout &  --  &  --  &  --  &    --  &    --  &     -- \\
\midrule
           &             &         28 &          3 &\textbf{29} & \textbf{99.5} & 93.4 & 87.6 &    \textbf{0.1} &  6.03  & 1996.1 \\
           &             & \multicolumn{3}{c|}{success frequency} & \multicolumn{3}{c|}{median} & \multicolumn{3}{c}{median} \\
\bottomrule
\end{tabular}
\end{center}

==> tables/acasxu-repair.tex <==
\renewcommand{\unknown}{?}

\begin{table}
    \scriptsize
    \centering
    \begin{tabular}{@{}cc|c@{ \,}cc@{\hskip 5pt}| c@{ \,}cc@{\hskip 5pt}| ccc@{} }\toprule
                 &       & \multicolumn{3}{c|}{\textbf{Repair Accuracy}} & \multicolumn{3}{c|}{\textbf{Repair MAE}} & \multicolumn{3}{c}{\textbf{\;Counter-ex. confidence}} \\
        Spec & Model\; & \;\tool{ } & DL2 & NF & \;\tool{ } & DL2 & NF & \;\tool{ } & DL2 & NF  \\ \midrule
        \multirow{32}{0.2cm}{$\varphi_2$}  
        & $N_{2,1}$ & \textbf{99.1}  & 21.1           & 83.9          & \textbf{0.22} & 0.77           & 9.08       & \textbf{6.9}   & 7.4          & 14.8   \\
        & $N_{2,2}$ & \textbf{98.7}  & 96.8           & \fail         & \textbf{0.23} & 0.37           & \fail      & \textbf{5.2}   & \textbf{5.2} & 16.5 \\
        & $N_{2,3}$ & \textbf{99.3}  & 97.6           & 83.5          & \textbf{0.13} & 0.19           & 26.55      & 6.5            & \textbf{3.9} & 12.3 \\
        & $N_{2,4}$ & \textbf{99.5}  & 99.1           & 83.6          & \textbf{0.09} & 0.14           & 2335.63    & \textbf{0.6}   & \textbf{0.6} & 1.0 \\
        & $N_{2,5}$ & \timeout       & 30.4           & \textbf{84.1} & \timeout      & \textbf{0.42}  & 1023.09    & \textbf{1.6}   & 4.0          & 9.7 \\
        & $N_{2,6}$ & \timeout       & \textbf{97.1}  & 85.6          & \timeout      & \textbf{0.15}  & 1501.14    & \textbf{0.3}   & 1.0          & 2.0 \\ 
        & $N_{2,7}$ & 14.5           & 14.8           & \textbf{14.9} & \textbf{0.15} & 0.25           & 0.41       & \textbf{4.0}   & 4.6          & 11.3 \\
        & $N_{2,8}$ & \textbf{99.6}  & 29.6           & \fail         & \textbf{0.14} & 0.78           & \fail      & \textbf{11.5}  & \textbf{11.5}& 18.6 \\
        & $N_{2,9}$ & \textbf{99.8}  & 99.2           & 88.6          & \textbf{0.13} & 0.22           & 1211.91    & \textbf{0.5}   & 0.8          & 2.4 \\
        & $N_{3,1}$ & \textbf{98.6}  & 80.9           & 8.8           & \textbf{0.27} & 0.57           & 3.23       & 8.1            & \textbf{6.8} & 14.4 \\
        & $N_{3,2}$ & \textbf{99.9}  & 99.8           & 86.5          & \textbf{0.10} & 0.13           & 2378.94    & \textbf{0.1}   & \textbf{0.1} & 0.4 \\
        & $N_{3,4}$ & \textbf{99.5}  & 98.3           & 83.7          & \textbf{0.10} & 0.23           & 127.51     & 9.5            & \textbf{5.9} & 12.0 \\
        & $N_{3,5}$ & \textbf{99.5}  & 32.4           & 84.2          & \textbf{0.09} & 0.38           & 2441.65    & \textbf{7.6}   & 8.0          & 14.0 \\
        & $N_{3,6}$ & \unknown       & 79.5           & \textbf{81.8} & \unknown      & 0.21           & 2410.51    & \textbf{0.3}   & 0.8          & 0.5 \\
        & $N_{3,7}$ & \textbf{99.7}  & 96.8           & \fail         & \textbf{0.11} & 0.30           & \fail      & 6.6            & \textbf{5.2} & 21.7 \\
        & $N_{3,8}$ & \textbf{99.7}  & \fail          & 87.9          & \textbf{0.09} & \fail          & 1024.48    & \textbf{1.3}   & 1.9          & 5.5 \\
        & $N_{3,9}$ & \timeout       & \textbf{88.4}  & \fail         & \timeout      & \textbf{0.48}  & \fail      & \textbf{5.1}   & 16.2         & 31.3 \\
        & $N_{4,1}$ & \textbf{99.8}  & 99.5           & 87.7          & \textbf{0.11} & 0.14           & 1564.80    & \textbf{1.3}   & \textbf{1.3} & 1.6 \\
        & $N_{4,3}$ & \textbf{99.4}  & 98.7           & 9.6           & \textbf{0.13} & 0.22           & 1.96       & \textbf{4.4}   & 5.3          & 10.6 \\
        & $N_{4,4}$ & \textbf{99.5}  & 98.7           & 10.4          & \textbf{0.10} & 0.20           & 1.03       & \textbf{6.6}   & 6.9          & 12.5 \\
        & $N_{4,5}$ & \textbf{99.4}  & 98.5           & 12.1          & \textbf{0.08} & 0.18           & 2.22       & 6.3            & \textbf{5.1} & 10.4 \\
        & $N_{4,6}$ & \textbf{99.6}  & 96.5           & 10.2          & \textbf{0.07} & 0.35           & 2.68       & \textbf{2.7}   & 4.3          & 14.1 \\
        & $N_{4,7}$ & \textbf{98.3}  & 62.0           & 88.9          & \textbf{0.14} & 0.57           & 33.47      & \textbf{3.0}   & 4.2          & 6.0 \\
        & $N_{4,8}$ & \textbf{99.1}  & 95.5           & \fail         & \textbf{0.16} & 0.27           & \fail      & 22.3           & \textbf{15.1}& 35.2 \\
        & $N_{4,9}$ & \textbf{99.5}  & 90.9           & 88.9          & \textbf{0.06} & 0.29           & 2438.07    & \textbf{0.4}   & \textbf{0.4} & 0.6 \\
        & $N_{5,1}$ & \textbf{99.5}  & 98.5           & 87.5          & \textbf{0.11} & 0.46           & 11.87      & \textbf{3.1}   & 5.0          & 7.1 \\
        & $N_{5,2}$ & \textbf{99.7}  & 98.9           & 87.6          & \textbf{0.10} & 0.25           & 845.28     & \textbf{2.2}   & \textbf{2.2} & 2.4 \\
        & $N_{5,4}$ & \textbf{99.6}  & 99.2           & 87.8          & \textbf{0.09} & 0.13           & 1064.02    & 3.6            & \textbf{3.4} & 9.3 \\
        & $N_{5,5}$ & \timeout       & \textbf{99.3}  & 10.8          & \timeout      & \textbf{0.15}  & 1.12       & \textbf{1.7}   & 4.5          & 8.4 \\
        & $N_{5,6}$ & \textbf{99.5}  & 98.9           & 89.6          & \textbf{0.12} & 0.16           & 526.73     & 1.3            & \textbf{1.2} & 3.1 \\
        & $N_{5,7}$ & \textbf{98.1}  & 90.8           & \fail         & \textbf{0.16} & 0.30           & \fail      & \textbf{4.2}   & 5.1          & 16.5 \\
        & $N_{5,8}$ & \textbf{99.4}  & 15.0           & 87.7          & \textbf{0.11} & 0.97           & 1871.85    & \textbf{6.2}   & 10.9         & 9.1 \\
        & $N_{5,9}$ & \textbf{98.1}  & 80.6           & 87.9          & \textbf{0.13} & 0.42           & 1977.43    & 6.3            & \textbf{4.7} & 12.8 \\
        $\varphi_7$                     
        & $N_{1,9}$ & \unknown        & \fail          & \textbf{0.04} & \unknown       & \fail  & \textbf{400.22}  & 0.1            & 0.2          & \textbf{0.0}\\
        $\varphi_8$                     
        & $N_{2,9}$ & \timeout        & \timeout        & \textbf{88.6} & \timeout       & \timeout & \textbf{32.86} & \textbf{0.0}  & \textbf{0.0} & \textbf{0.0}\\
        $\Phi_1$                     
        & $N_{2,9}$ & \timeout        & \unknown        & \fail         & \timeout        & \unknown    & \fail      & 1.2           & \textbf{1.0} & 3029.7\\
        \midrule
        \multicolumn{2}{@{}l|}{\#successes}  & 28 & \textbf{32} & 29 \\
        \multicolumn{2}{@{}l|}{median}        & \textbf{99.5} & 96.8 & 84.2   & \textbf{0.11} & 0.26 & 526.73 & \textbf{3.35} & 4.4 & 10.05 \\
        \bottomrule
    \end{tabular}
    \caption{\textbf{Safety repair results of the ACAS Xu DNNs}: \tool{ } (this work), DL2, and neuron fixation. \timeout{ }indicates a timeout, `\unknown' marks cases where the verifier returned \textsc{unknown}, and \fail{ }indicates unsuccessful repairs.}
    \label{tab:repair-acas-xu}
\end{table}

==> tables/min-cx-severity-experiments/repair-cifar10-min-cx.tex <==
\begin{table}
\begin{tabular}{@{}ccllllllllll@{}}
\toprule
       &       &                     &                 &            &                 & \multicolumn{3}{c}{Test Acc. (\%)} & \multicolumn{3}{c}{Train Acc. (\%)} \\
Points & Cases & \(\#_{\exsuccess}\) & \(\#_{\exfailure}\) & \(\#_{\exunknown}\) & \(\#_{\extimeout}\) & min  & med  & max & min  & max  & max  \\
\midrule
1 & 100 &  96 &   2 &   0 &   2 & 50.6 & 68.8 & 70.7 & 58.7 & 90.1 & 95.0 \\
25 & 4 & \multicolumn{4}{c}{\(\exsuccess, \exfailure, \exfailure, \exunknown\)} & \multicolumn{3}{c}{69.2} & \multicolumn{3}{c}{92.8} \\
100 & 1 & \multicolumn{4}{c}{ -- } & \multicolumn{3}{c}{ -- } & \multicolumn{3}{c}{ -- } \\
\bottomrule
\end{tabular}

\caption{\textbf{\tool{ }}}
\caption[Repairing Robustness of Convolutional Image Classifiers: Repair Outcomes]{\textbf{Repairing Robustness of Convolutional Image Classifiers using Minimal Severity Counter-Examples: Repair Outcomes}. 
A \(\color{Set1-A}{\timeout{}}\) indicates that exceeding the three-hour time limit was only discovered after repair. 
When incorporating the timeouts discovered during analysis, the \tool{ } repair algorithm successfully repairs violations of specification concerned with a single data point only \num{74} times, while there are \num{20} timeouts. 
}
\label{tab:experiments-cifar10-min-cx-results}
\end{table}

==> tables/min-cx-severity-experiments/repair-mnist-min-cx.tex <==

\begin{table}

\begin{tabular}{@{}cclllllll@{}}
\toprule
       &       &                     &                     &                     &                     & \multicolumn{3}{c}{Test Acc. (\%)} \\
Points & Cases & \(\#_{\exsuccess}\) & \(\#_{\exfailure}\) & \(\#_{\exunknown}\) & \(\#_{\extimeout}\) & min  & med  & max \\
\midrule
1 & 100 &  99 &   0 &   1 &   0 & 92.9 & 96.4 & 97.3 \\
10 & 10 &   7 &   0 &   3 &   0 & 96.4 & 96.9 & 97.3 \\
25 & 4 & \multicolumn{4}{c}{\(\exsuccess, \exunknown_{\color{Set1-A}{\extimeout{}}}, \exunknown_{\color{Set1-A}{\extimeout{}}}, \exunknown_{\color{Set1-A}{\extimeout{}}}\)} & \multicolumn{3}{c}{97.3} \\
50 & 2 & \multicolumn{4}{c}{\(\exunknown_{\color{Set1-A}{\extimeout{}}}, \exunknown_{\color{Set1-A}{\extimeout{}}}\)} & \multicolumn{3}{c}{ -- } \\
100 & 1 & \multicolumn{4}{c}{\(\extimeout\)} & \multicolumn{3}{c}{ -- } \\
\bottomrule
\end{tabular}
\caption{\textbf{Repairing Robustness of a DiffAI-Defended MNIST Network using Minimal Severity Counter-Examples:} Repair outcome for \tool{ }.}
\label{tab:experiment-min-cx-mnist-results}
\end{table}

==> tables/repair-cifar10-full.tex <==
\begin{table}
\scriptsize
\begin{subtable}[t]{\textwidth}
\centering
\begin{tabular}{@{}ccllllllllll@{}}
\toprule
       &       &                     &                 &            &                 & \multicolumn{3}{c}{Test Acc. (\%)} & \multicolumn{3}{c}{Train Acc. (\%)} \\
Points & Cases & \(\#_{\success}\) & \(\#_{\fail}\) & \(\#_{\exunknown}\) & \(\#_{\timeout}\) & min  & med  & max & min  & max  & max  \\
\midrule
1 & 100 &  \(88_{\color{Set1-A}{\timeout{}} 14}\) &   5 &   1 &   6 & 62.3 & \textbf{69.6} & 70.7 & 75.7 & \textbf{92.5} & 95.6 \\
25 & 4 & \multicolumn{4}{c}{\(\success_{\color{Set1-A}{\timeout{}}}, \fail, \timeout, \timeout\)} & \multicolumn{3}{c}{\textbf{69.1}} & \multicolumn{3}{c}{\textbf{86.7}} \\
100 & 1 & \multicolumn{4}{c}{\(\fail\)} & \multicolumn{3}{c}{ -- } & \multicolumn{3}{c}{ -- } \\
\bottomrule
\end{tabular}
\caption{\textbf{\tool{ } Repair}}
\end{subtable}
%
\begin{subtable}[t]{\textwidth}
\centering
\begin{tabular}{@{}ccllllllllll@{}}
\toprule
       &       &                     &                 &            &                 & \multicolumn{3}{c}{Test Acc. (\%)} & \multicolumn{3}{c}{Train Acc. (\%)} \\
Points & Cases & \(\#_{\success}\) & \(\#_{\fail}\) & \(\#_{\exunknown}\) & \(\#_{\timeout}\) & min  & med  & max & min  & max  & max  \\
\midrule
1 & 100 &  93 &   7 &   0 &   0 & 65.4 & 69.3 & 70.3 & 82.8 & 91.9 & 93.9 \\
25 & 4 & \multicolumn{4}{c}{\(\fail, \fail, \fail, \fail\)} & \multicolumn{3}{c}{ -- } & \multicolumn{3}{c}{ -- } \\
100 & 1 & \multicolumn{4}{c}{\(\timeout\)} & \multicolumn{3}{c}{ -- } & \multicolumn{3}{c}{ -- } \\
\bottomrule
\end{tabular}
\caption{\textbf{DL2 Repair}}
\end{subtable}
%
\begin{subtable}[t]{\textwidth}
\centering
\begin{tabular}{@{}ccllllllllll@{}}
\toprule
       &       &                     &                 &            &                 & \multicolumn{3}{c}{Test Acc. (\%)} & \multicolumn{3}{c}{Train Acc. (\%)} \\
Points & Cases & \(\#_{\success}\) & \(\#_{\fail}\) & \(\#_{\exunknown}\) & \(\#_{\timeout}\) & min  & med  & max & min  & max  & max  \\
\midrule
1 & 100 &  77 &  23 &   0 &   0 & 30.4 & 48.4 & 51.0 & 36.0 & 55.8 & 59.2 \\
25 & 4 & \multicolumn{4}{c}{\(\fail, \fail, \fail, \fail\)} & \multicolumn{3}{c}{ -- } & \multicolumn{3}{c}{ -- } \\
100 & 1 & \multicolumn{4}{c}{\(\fail\)} & \multicolumn{3}{c}{ -- } & \multicolumn{3}{c}{ -- } \\
\bottomrule
\end{tabular}
\caption{\textbf{Minimal Modification Repair}}
\end{subtable}
\caption[Repairing Robustness of Convolutional Image Classifiers: Repair Outcomes]{\textbf{Repairing Robustness of Convolutional Image Classifiers: Repair Outcomes}. 
A \(\color{Set1-A}{\timeout{}}\) indicates that exceeding the three-hour time limit was only discovered after repair. 
When incorporating the timeouts discovered during analysis, the \tool{ } repair algorithm successfully repairs violations of specification concerned with a single data point only \num{74} times, while there are \num{20} timeouts. 
}
\label{tab:experiments-cifar10-results}
\end{table}

==> tables/repair-mnist-defended-full.tex <==

\begin{table}
\scriptsize
\centering
\begin{subtable}[t]{0.49\textwidth}
\centering
\begin{tabular}{@{}cclllllll@{}}
\toprule
       &       &                     &                     &                     &                     & \multicolumn{3}{c}{Test Acc. (\%)} \\
Points & Cases & \(\#_{\success}\) & \(\#_{\fail}\) & \(\#_{\exunknown}\) & \(\#_{\timeout}\) & min  & med  & max \\
\midrule
1 & 100 & 100 &   0 &   0 &   0 & 95.4 & \textbf{96.3} & 96.7 \\
10 & 10 &  10 &   0 &   0 &   0 & 95.8 & 96.1 & 96.4 \\
25 & 4 & \multicolumn{4}{c}{\(\success, \success, \success, \success\)} & 94.9 & \textbf{96.4} & 96.8 \\
50 & 2 & \multicolumn{4}{c}{\(\success_{\color{Set1-A}{\timeout{}}}, \timeout\)} & \multicolumn{3}{c}{\textbf{96.8}} \\
100 & 1 & \multicolumn{4}{c}{\(\success_{\color{Set1-A}{\timeout{}}}\)} & \multicolumn{3}{c}{\textbf{95.4}} \\
\bottomrule
\end{tabular}
\caption[\tool{ } Repair]{\textbf{\tool{ } Repair}}
\end{subtable} %
%
\begin{subtable}[t]{0.5\textwidth}
\centering
\begin{tabular}{@{}cclllllll@{}}
\toprule
       &       &                     &                     &                     &                     & \multicolumn{3}{c}{Test Acc. (\%)} \\
Points & Cases & \(\#_{\success}\) & \(\#_{\fail}\) & \(\#_{\exunknown}\) & \(\#_{\timeout}\) & min  & med  & max \\
\midrule
1 & 100 & 100 &   0 &   0 &   0 & 95.7 & 96.2 & 96.7 \\
10 & 10 &   8 &   0 &   0 &   2 & 95.3 & \textbf{96.2} & 96.5 \\
25 & 4 & \multicolumn{4}{c}{\(\timeout, \timeout, \timeout, \timeout\)} & \multicolumn{3}{c}{ -- } \\
50 & 2 & \multicolumn{4}{c}{\(\timeout, \timeout\)} & \multicolumn{3}{c}{ -- } \\
100 & 1 & \multicolumn{4}{c}{\(\timeout\)} & \multicolumn{3}{c}{ -- } \\
\bottomrule
\end{tabular}
\caption[DL2 Repair]{\textbf{DL2 Repair}}
\end{subtable}

\begin{subtable}[t]{0.5\textwidth}
\centering
\begin{tabular}{@{}cclllllll@{}}
\toprule
       &       &                     &                     &                     &                     & \multicolumn{3}{c}{Test Acc. (\%)} \\
Points & Cases & \(\#_{\success}\) & \(\#_{\fail}\) & \(\#_{\exunknown}\) & \(\#_{\timeout}\) & min  & med  & max \\
\midrule
1 & 100 & 100 &   0 &   0 &   0 & 89.1 & 95.8 & 96.0 \\
10 & 10 &  10 &   0 &   0 &   0 & 81.4 & 90.3 & 94.7 \\
25 & 4 & \multicolumn{4}{c}{\(\success, \success, \success, \success\)} & 75.3 & 86.1 & 91.2 \\
50 & 2 & \multicolumn{4}{c}{\(\success, \timeout\)} & \multicolumn{3}{c}{80.6} \\
100 & 1 & \multicolumn{4}{c}{\(\fail\)} & \multicolumn{3}{c}{ -- } \\
\bottomrule
\end{tabular}
\caption{\textbf{Minimal Modification Repair}}
\end{subtable}%
%
\begin{subtable}[t]{0.5\textwidth}
\centering
\begin{tabular}{@{}cclllllll@{}}
\toprule
       &       &                     &                     &                     &                     & \multicolumn{3}{c}{Test Acc. (\%)} \\
Points & Cases & \(\#_{\success}\) & \(\#_{\fail}\) & \(\#_{\exunknown}\) & \(\#_{\timeout}\) & min  & med  & max \\
\midrule
1 & 100 &  75 &  25 &   0 &   0 & 80.6 & 95.3 & 96.0 \\
10 & 10 &   0 &  10 &   0 &   0 & \multicolumn{3}{c}{ -- } \\
25 & 4 & \multicolumn{4}{c}{\(\fail, \fail, \fail, \fail\)} & \multicolumn{3}{c}{ -- } \\
50 & 2 & \multicolumn{4}{c}{\(\fail, \fail\)} & \multicolumn{3}{c}{ -- } \\
100 & 1 & \multicolumn{4}{c}{\(\fail\)} & \multicolumn{3}{c}{ -- } \\
\bottomrule
\end{tabular}
\caption{\textbf{Neuron Fixation Repair}}
\end{subtable}
\caption{\textbf{Repairing Robustness of a DiffAI-Defended MNIST Network:} Repair Outcomes.}
\label{tab:experiments-mnist-results}
\end{table}

==> tables/specification-satisfaction.tex <==
\begin{table*}[t]
    \scriptsize
    \begin{center}
        \begin{tabular}{@{}c|l|rr|rr|rr@{}}
        \toprule
        \multirow{2}{*}{Spec} &  \multirow{2}{*}{Models} & \multicolumn{2}{c|}{\textbf{Ground Truth}} & \multicolumn{2}{c|}{\textbf{naïve \tool{ }}} & \multicolumn{2}{c}{\textbf{\tool{ }}}  \\ 
        & & \#\sat & \#\unsat  & \#\sat & \#$\unknown$ & \#\sat & \#$\unknown$  \\
        \midrule
        $\varphi_1$ & all                      & 0  & 45 &  0           & 45         & 0           & 45            \\
        $\varphi_2$ & $N_{2,1}$ to $N_{5,9}$    & 35 & 1  &  \textbf{30} & \textbf{6} & \textbf{35} & \textbf{1}    \\
        $\varphi_3$ & all except $N_{1,7}$ to $N_{1,9}$ & 0  & 42 &  0           & 42         & 0           & 42            \\
        $\varphi_4$ & all except $N_{1,7}$ to $N_{1,9}$ & 0  & 42 &  0           & 42         & 0           & 42            \\
        $\varphi_5$ & $N_{1,1}$                 & 0  & 1  &  0           & 1          & 0           & 1             \\
        $\varphi_6$ & $N_{1,1}$                 & 0  & 1  &  0           & 1          & 0           & 1             \\
        $\varphi_7$ & $N_{1,9}$                 & 1  & 0  &  \textbf{0}  & \textbf{1} & \textbf{1}  & \textbf{0}    \\
        $\varphi_8$ & $N_{2,9}$                 & 1  & 0  &  \textbf{0}  & \textbf{1} & \textbf{1}  & \textbf{0}    \\
        $\varphi_9$ & $N_{3,3}$                 & 0  & 1  &  0           & 1          & 0           & 1             \\
        $\varphi_{10}$ & $N_{4,5}$                & 0  & 1  &  0           & 1          & 0           & 1             \\
        \bottomrule
    \end{tabular}
    
    \caption{
        \textbf{ Safety specification compliance analysis of the ACAS Xu DNNs}: Conducted on networks $N_{1,1}$ to $N_{5,9}$, a total of 45 networks \protect\citep{DBLP:conf/cav/KatzBDJK17}. 
        We compare naïve \tool{ }, and \tool{ } (this work).
        Some properties apply to all networks, while others apply only to a subset of these networks (second column).
        The ground truth is obtained using ERAN \cite{DBLP:journals/pacmpl/SinghGPV19}. $\sat$\ means that the specification is violated, i.e., a counter-example exists.
        The numbers in bold mark a difference between naïve \tool{ } and \tool{ }.
        }
    \label{table:acas-xu-specattack}
    \end{center}
\end{table*}
